Engineering Pitfalls in AI Coding Tools: An Empirical Study of Bugs in Claude Code, Codex, and Gemini CLI

The rapid integration of Large Language Models (LLMs) into software development workflows has given rise to a new class of AI-assisted coding tools, such as Claude-Code, Codex, and Gemini CLIs. While promising significant productivity gains, the engineering process of building these tools, which sit at the complex intersection of traditional software engineering, AI system design, and human-computer interaction, is fraught with unique and poorly understood challenges. This paper presents the first empirical study of engineering pitfalls in building such tools, on a systematic, manual analysis of over 3.8K publicly reported bugs in the open-source repositories of three AI-assisted coding tools (i.e., Claude-Code, Codex, and Gemini CLIs) on GitHub. Specifically, we employ an open-coding methodology to manually examine the issue description, associated user discussions, and developer responses. Through this process, we categorize each bug along multiple dimensions, including bug type, bug location, root cause, and observed symptoms. This fine-grained annotation enables us to characterize common failure patterns and identify recurring engineering challenges. Our results show that more than 67% of the bugs in these tools are related to functionality. In terms of root causes, 36.9% of the bugs stem from API, integration, or configuration errors. Consequently, the most commonly observed symptoms reported by users are API errors (18.3%), terminal problems (14%), and command failures (12.7%). These bugs predominantly affect the tool invocation (37.2%) and command execution (24.7%) stages of the system workflow. Collectively, our findings provide a critical roadmap for developers seeking to design the next generation of reliable and robust AI coding assistants.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> figure/dist_bug_impact.tex <==
\begin{figure}[t!]
  \centering
  \begin{tikzpicture}
    \pgfplotsset{compat=1.18}

    \begin{axis}[
     font=\scriptsize,
      ybar stacked,
      width=\linewidth,
      height=5cm,
      bar width=20pt,
      ymin=0,
      enlarge x limits=0.10,
      xlabel={Architectural Layer},
      ylabel={Bug Count},
      symbolic x coords={
        Orchestration,
        Exec,
        UI,
        State,
        LLM,
        Prompt
      },
      xticklabels={
        {Tool/API Orchestration},
        {Command Execution \& Monitoring},
        {User Interface \& Interaction},
        {State \& Memory Management},
        {LLM Reasoning Planning},
        {Prompt Engineering \& Context Management}
      },
      xtick=data,
      xticklabel style={
        rotate=45,
        anchor=east,
        font=\small,
        align=center,
        text width=3cm
      },
      legend style={
        at={(0.80,0.98)},
        anchor=north east,
        draw=gray!40,
        fill=white,
        font=\small
      },
      ymajorgrids=true,
      grid style={opacity=0.25},
      nodes near coords,
      nodes near coords style={
        font=\scriptsize,
        color=white
      },
    ]

    % Claude Code (Blue)
    \addplot[fill=blue!60] coordinates {
      (Orchestration,940)
      (Exec,559)
      (UI,344)
      (State,225)
      (LLM,113)
      (Prompt,142)
    };

    % Codex CLI (Orange)
    \addplot[fill=orange!85] coordinates {
      (Orchestration,407)
      (Exec,332)
      (UI,207)
      (State,94)
      (LLM,111)
      (Prompt,40)
    };

    % Gemini CLI (Green)
    \addplot[fill=green!60] coordinates {
      (Orchestration,98)
      (Exec,68)
      (UI,75)
      (State,30)
      (LLM,22)
      (Prompt,35)
    };

    \legend{Claude Code, Codex CLI, Gemini CLI}

    % ---- TOP TOTAL LABELS ----
    \node[font=\small,anchor=south] at (axis cs:Orchestration,1445) {1445};
    \node[font=\small,anchor=south] at (axis cs:Exec,959) {959};
    \node[font=\small,anchor=south] at (axis cs:UI,626) {626};
    \node[font=\small,anchor=south] at (axis cs:State,349) {349};
    \node[font=\small,anchor=south] at (axis cs:LLM,246) {246};
    \node[font=\small,anchor=south] at (axis cs:Prompt,217) {217};

    \draw[->,thick] (axis cs:Orchestration,1400) -- (axis cs:Orchestration,1445);
    \draw[->,thick] (axis cs:Exec,915) -- (axis cs:Exec,959);
    \draw[->,thick] (axis cs:UI,585) -- (axis cs:UI,626);
    \draw[->,thick] (axis cs:State,315) -- (axis cs:State,349);
    \draw[->,thick] (axis cs:LLM,215) -- (axis cs:LLM,246);
    \draw[->,thick] (axis cs:Prompt,185) -- (axis cs:Prompt,217);

    \end{axis}
  \end{tikzpicture}
  \caption{Bug distribution across AI Coding architectural layers}
  \label{fig:bug_stage_distribution}
\end{figure}

==> figure/dist_bug_symptom.tex <==
\begin{figure*}[t!]
  \centering
  \begin{tikzpicture}
    \begin{axis}[
     font=\scriptsize,
      ybar stacked,
      bar width=13pt,
      width=\textwidth,
      height=5cm,
      ymin=0,
      enlarge x limits=0.06,
      ylabel={Count},
      xlabel={Symptom Category},
      symbolic x coords={
        {API \& Server Communication},
        {CLI/Terminal Experience},
        {Command Execution},
        {Code \& File Operations},
        {AI Model \& Output Control},
        {Authentication \& Access},
        {User Feedback \& Usability},
        {Session \& State Management},
        {Configuration \& State},
        {Installation \& Setup},
        {Security \& Data Management},
        {Integration \& Compatibility},
        {Model Selection \& Availability},
        {Hook \& Automation Issues},
        {Cost \& Billing},
        {Image \& Media Handling}
      },
      xtick=data,
      xticklabel style={rotate=50,anchor=east},
      yticklabel style={/pgf/number format/1000 sep=,},
      legend style={
        at={(0.97,0.97)},
        anchor=north east,
        draw=gray!40,
        fill=white,
        title=%placeholder
      },
    ]

    % Claude Code
    \addplot+[fill=blue!60,
      nodes near coords={\pgfmathprintnumber[1000 sep=,]{\pgfplotspointmeta}},
      nodes near coords style={font=\scriptsize, color=black, yshift=0pt}
    ] coordinates {
      ({API \& Server Communication},420)
      ({CLI/Terminal Experience},315)
      ({Command Execution},286)
      ({Code \& File Operations},168)
      ({AI Model \& Output Control},111)
      ({Authentication \& Access},129)
      ({User Feedback \& Usability},162)
      ({Session \& State Management},140)
      ({Configuration \& State},144)
      ({Installation \& Setup},120)
      ({Security \& Data Management},107)
      ({Integration \& Compatibility},68)
      ({Model Selection \& Availability},58)
      ({Hook \& Automation Issues},47)
      ({Cost \& Billing},26)
      ({Image \& Media Handling},22)
    };

    % Codex CLI
    \addplot+[fill=orange!85,
      nodes near coords={\pgfmathprintnumber[1000 sep=,]{\pgfplotspointmeta}},
      nodes near coords style={font=\scriptsize, color=black, yshift=0pt}
    ] coordinates {
      ({API \& Server Communication},245)
      ({CLI/Terminal Experience},154)
      ({Command Execution},164)
      ({Code \& File Operations},74)
      ({AI Model \& Output Control},132)
      ({Authentication \& Access},105)
      ({User Feedback \& Usability},57)
      ({Session \& State Management},68)
      ({Configuration \& State},49)
      ({Installation \& Setup},34)
      ({Security \& Data Management},16)
      ({Integration \& Compatibility},37)
      ({Model Selection \& Availability},35)
      ({Hook \& Automation Issues},0)
      ({Cost \& Billing},8)
      ({Image \& Media Handling},13)
    };

    % Gemini CLI
    \addplot+[fill=green!60,
      nodes near coords={\pgfmathprintnumber[1000 sep=,]{\pgfplotspointmeta}},
      nodes near coords style={font=\scriptsize, color=black, yshift=0pt}
    ] coordinates {
      ({API \& Server Communication},40)
      ({CLI/Terminal Experience},73) 
      ({Command Execution},40)
      ({Code \& File Operations},35)
      ({AI Model \& Output Control},27)
      ({Authentication \& Access},24)
      ({User Feedback \& Usability},21)
      ({Session \& State Management},16)
      ({Configuration \& State},15)
      ({Installation \& Setup},10)
      ({Security \& Data Management},5)
      ({Integration \& Compatibility},10)
      ({Model Selection \& Availability},3)
      ({Hook \& Automation Issues},5)
      ({Cost \& Billing},3)
      ({Image \& Media Handling},1)
    };

    \legend{Claude Code,Codex CLI,Gemini CLI}

    \node[font=\small,anchor=south] at (axis cs:API \& Server Communication,705) {705};
    \node[font=\small,anchor=south] at (axis cs:CLI/Terminal Experience,542) {542};
    \node[font=\small,anchor=south] at (axis cs:Command Execution,490) {490};
    \node[font=\small,anchor=south] at (axis cs:Code \& File Operations,277) {277};
    \node[font=\small,anchor=south] at (axis cs:AI Model \& Output Control,270) {270};
    \node[font=\small,anchor=south] at (axis cs:Authentication \& Access,258) {258};
    \node[font=\small,anchor=south] at (axis cs:User Feedback \& Usability,240) {240};
    \node[font=\small,anchor=south] at (axis cs:Session \& State Management,224) {224};
    \node[font=\small,anchor=south] at (axis cs:Configuration \& State,208) {208};
    \node[font=\small,anchor=south] at (axis cs:Installation \& Setup,164) {164};
    \node[font=\small,anchor=south] at (axis cs:Security \& Data Management,128) {128};
    \node[font=\small,anchor=south] at (axis cs:Integration \& Compatibility,115) {115};
    \node[font=\small,anchor=south] at (axis cs:Model Selection \& Availability,96) {96};
    \node[font=\small,anchor=south] at (axis cs:Hook \& Automation Issues,52) {52};
    \node[font=\small,anchor=south] at (axis cs:Cost \& Billing,37) {37};
    \node[font=\small,anchor=south] at (axis cs:Image \& Media Handling,36) {36};

    \draw[->,thick] (axis cs:API \& Server Communication,705) -- (axis cs:API \& Server Communication,705);
    \draw[->,thick] (axis cs:CLI/Terminal Experience,542) -- (axis cs:CLI/Terminal Experience,542);
    \draw[->,thick] (axis cs:Command Execution,490) -- (axis cs:Command Execution,490);
    \draw[->,thick] (axis cs:Code \& File Operations,277) -- (axis cs:Code \& File Operations,277);
    \draw[->,thick] (axis cs:AI Model \& Output Control,270) -- (axis cs:AI Model \& Output Control,270);
    \draw[->,thick] (axis cs:Authentication \& Access,258) -- (axis cs:Authentication \& Access,258);
    \draw[->,thick] (axis cs:User Feedback \& Usability,240) -- (axis cs:User Feedback \& Usability,240);
    \draw[->,thick] (axis cs:Session \& State Management,224) -- (axis cs:Session \& State Management,224);
    \draw[->,thick] (axis cs:Configuration \& State,208) -- (axis cs:Configuration \& State,208);
    \draw[->,thick] (axis cs:Installation \& Setup,164) -- (axis cs:Installation \& Setup,164);
    \draw[->,thick] (axis cs:Security \& Data Management,128) -- (axis cs:Security \& Data Management,128);
    \draw[->,thick] (axis cs:Integration \& Compatibility,115) -- (axis cs:Integration \& Compatibility,115);
    \draw[->,thick] (axis cs:Model Selection \& Availability,96) -- (axis cs:Model Selection \& Availability,96);
    \draw[->,thick] (axis cs:Hook \& Automation Issues,52) -- (axis cs:Hook \& Automation Issues,52);
    \draw[->,thick] (axis cs:Cost \& Billing,37) -- (axis cs:Cost \& Billing,37);
    \draw[->,thick] (axis cs:Image \& Media Handling,36) -- (axis cs:Image \& Media Handling,36);

    \end{axis}
  \end{tikzpicture}
  \caption{Distribution of symptom categories by model.}
  \label{fig:symptom-category-by-model}
\end{figure*}

==> figure/dist_bug_types.tex <==
\begin{figure}[t!]
  \centering
  \begin{tikzpicture}
    \begin{axis}[
    font=\scriptsize,
      ybar stacked,
      bar width=15pt,
      width=\linewidth,
      height=5cm,
      ymin=0,
      enlarge x limits=0.06,
      ylabel={Count},
      xlabel={Bug Type},
      symbolic x coords={Functional Bugs,Usability Bugs,Compatibility Bugs,UI Bugs,Performance Bugs,Security Bugs},
      xtick=data,
      xticklabel style={rotate=35,anchor=east},
      yticklabel style={/pgf/number format/1000 sep=,},
      legend style={
        at={(0.95,0.95)},
        anchor=north east,
        draw=gray!40,
        fill=white,
        title=%placeholder
      },
    ]
    % Stacked bars
    \addplot+[fill=blue!60,
      nodes near coords={\pgfmathprintnumber[1000 sep=,]{\pgfplotspointmeta}},
      nodes near coords style={font=\scriptsize, color=black, yshift=0pt}] coordinates {
      (Functional Bugs,1555) (Usability Bugs,257)(Compatibility Bugs,147)
      (UI Bugs,160) (Performance Bugs,167)(Security Bugs,37)
};

    \addplot+[fill=orange!85,
      nodes near coords={\pgfmathprintnumber[1000 sep=,]{\pgfplotspointmeta}},
      nodes near coords style={font=\scriptsize, color=black, yshift=0pt}
      ] coordinates {
      (Functional Bugs,794) (Usability Bugs,115) (Compatibility Bugs,117)
       (UI Bugs,105)(Performance Bugs,38) (Security Bugs,22)
};

    \addplot+[fill=green!60,
        nodes near coords={\pgfmathprintnumber[1000 sep=,]{\pgfplotspointmeta}},
        nodes near coords style={font=\scriptsize, yshift=0pt}
        ] coordinates {
        (Functional Bugs,225) (Usability Bugs,31)
        (Compatibility Bugs,30) (UI Bugs,16) (Performance Bugs,19) (Security Bugs,7)
};
    \legend{Claude Code,Codex CLI,Gemini CLI}
    \node[font=\small,anchor=south] at (axis cs:Functional Bugs,2574) {2574};
    \node[font=\small,anchor=south] at (axis cs:Usability Bugs,403) {403};
    \node[font=\small,anchor=south] at (axis cs:Compatibility Bugs,294) {294};
    \node[font=\small,anchor=south] at (axis cs:UI Bugs,281) {281};
    \node[font=\small,anchor=south] at (axis cs:Performance Bugs,224) {224};
    \node[font=\small,anchor=south] at (axis cs:Security Bugs,66) {66};
    

    \draw[->,thick] (axis cs:Functional Bugs,2574) -- (axis cs:Functional Bugs,2574);
    \draw[->,thick] (axis cs:Usability Bugs,403) -- (axis cs:Usability Bugs,403);
    \draw[->,thick] (axis cs:Compatibility Bugs,294) -- (axis cs:Compatibility Bugs,294);
    \draw[->,thick] (axis cs:UI Bugs,281) -- (axis cs:UI Bugs,281);
    \draw[->,thick] (axis cs:Performance Bugs,224) -- (axis cs:Performance Bugs,224);
    \draw[->,thick] (axis cs:Security Bugs,66) -- (axis cs:Security Bugs,66);
    \end{axis}
  \end{tikzpicture}
  \vspace{-0.1in}
  \caption{Distribution of bug types by tool.
  \hung{Need a better way to show the number. Hard to read. Also, need a consistent color of number between figure. Not sure if this kind of figures is giving too much. Considering pie charts? The differences in the number of bugs between tools make it hard to see the most important distribution between categories. Maybe 3 pie charts instead?}
  }
  \label{fig:bugtype-by-model}
\end{figure}

==> figure/rootcs.tex <==
\begin{figure}[t!]
  \centering
  \begin{tikzpicture}
    \pgfplotsset{compat=1.18}

    \begin{axis}[
     font=\scriptsize,
      ybar stacked,
      width=\linewidth,
      height=5cm,
      bar width=15pt,
 ymin=0,
      enlarge x limits=0.10,
      xlabel={Root Cause Category},
    %  xlabel style={yshift=-3mm},   % <-- move xlabel closer to axis
      ylabel={Count},
    %  ylabel style={yshift=0mm},
      symbolic x coords={
        API,
        Config,
        UI,
        Env,
        {AI Logic},
        Perf,
        Exec,
        State,
        Code,
        Security
      },
      xticklabels={
        API,
        Config,
        UI,
        Env.,
       {AI Logic},
        Perf.,
        Exec.,
        State,
        Code,
        Security
    %    {API \& Integration Errors},
     %   {Configuration \& Setup},
     %   {User Interaction \& UI},
     %   {Environment \& Platform Compatibility},
      %  {AI Logic \& Behavior},
      %  {Performance \& Resource Limits},
      %  {Command Execution \& Parsing},
      %  {State \& Context Management},
      %  {Code \& File Handling},
      %  {Permissions \& Security}
      },
      xtick=data,
      xticklabel style={
        rotate=60,
        anchor=east,
        font=\small,
        align=right,
       % text width=5cm
      },
      legend style={
        at={(0.80,0.98)},
        anchor=north east,
        draw=gray!40,
        fill=white,
        font=\small
      },
      ymajorgrids=true,
      grid style={opacity=0.25},
      nodes near coords,
      nodes near coords style={
        font=\scriptsize,
        color=white
      },
    ]

    % Claude Code (Blue)
    \addplot[fill=blue!60] coordinates {
      (API,492)
      (Config,435)
      (UI,229)
      (Env,231)
      (AI Logic,158)
      (Perf,195)
      (Exec,179)
      (State,170)
      (Code,142)
      (Security,92)
    };

    % Codex CLI (Orange)
    \addplot[fill=orange!85] coordinates {
      (API,282)
      (Config,134)
      (UI,137)
      (Env,130)
      (AI Logic,183)
      (Perf,92)
      (Exec,64)
      (State,65)
      (Code,47)
      (Security,57)
    };

    % Gemini CLI (Green)
    \addplot[fill=green!60] coordinates {
      (API,49)
      (Config,41)
      (UI,61)
      (Env,43)
      (AI Logic,43)
      (Perf,21)
      (Exec,18)
      (State,17)
      (Code,25)
      (Security,10)
    };

    \legend{Claude Code, Codex CLI, Gemini CLI}

    % ---- TOP TOTAL LABELS ----
    \node[font=\small,anchor=south] at (axis cs:API,823) {823};
    \node[font=\small,anchor=south] at (axis cs:Config,610) {610};
    \node[font=\small,anchor=south] at (axis cs:UI,427) {427};
    \node[font=\small,anchor=south] at (axis cs:Env,404) {404};
    \node[font=\small,anchor=south] at (axis cs:{AI Logic},384) {384};
    \node[font=\small,anchor=south] at (axis cs:Perf,308) {308};
    \node[font=\small,anchor=south] at (axis cs:Exec,261) {261};
    \node[font=\small,anchor=south] at (axis cs:State,252) {252};
    \node[font=\small,anchor=south] at (axis cs:Code,214) {214};
    \node[font=\small,anchor=south] at (axis cs:Security,159) {159};

    \draw[->,thick] (axis cs:API,780) -- (axis cs:API,823);
    \draw[->,thick] (axis cs:Config,575) -- (axis cs:Config,610);
    \draw[->,thick] (axis cs:UI,395) -- (axis cs:UI,427);
    \draw[->,thick] (axis cs:Env,370) -- (axis cs:Env,404);
    \draw[->,thick] (axis cs:{AI Logic},350) -- (axis cs:Logic,384);
    \draw[->,thick] (axis cs:Perf,275) -- (axis cs:Perf,308);
    \draw[->,thick] (axis cs:Exec,235) -- (axis cs:Exec,261);
    \draw[->,thick] (axis cs:State,225) -- (axis cs:State,252);
    \draw[->,thick] (axis cs:Code,190) -- (axis cs:Code,214);
    \draw[->,thick] (axis cs:Security,135) -- (axis cs:Security,159);

    \end{axis}
  \end{tikzpicture}
  \caption{Distribution of root cause categories across tools
  \hung{The top number is hard to read in some of the smaller categories. Also there are some lines between the first 5 categories!}
  }
  \label{fig:root_cause_distribution}
\end{figure}

==> sections/new.tex <==
\section{Lesson Learned}
\label{sec:dis} 
Our study reveals several interesting findings that can serve
as practical guidelines for both industry and academic communities to improve AI coding tool development and testing in the future. 

\subsection{System-Level Failures Dominate}
Our empirical results suggest that many failures in AI coding tools stem from weak coordination between the language model, the supporting tool infrastructure, and the execution environment, rather than from model reasoning alone. This is reflected in the root cause distribution in Section~\ref{4.2}, where \textit{API \& Integration Errors} (21.4\%), together with \textit{Configuration \& Setup} issues (15.9\%), account for a large portion of observed failures. These root causes typically occur at system boundaries, such as API mismatches, authentication, network conditions, environment variables, path resolution, and version compatibility. 
Moreover, failures categorized under \textit{AI Logic \& Behaviour}, which represent intrinsic model-level issues such as instruction noncompliance or hallucinated outputs, account for a smaller portion of the dataset (10.0\%), as shown in Table~\ref{tab:root_cause_taxonomy}. This relatively small share may partially reflect reporting bias from a user perspective: developers are more likely to report failures that severely disrupt or block their normal workflows (e.g., tool crashes, execution failures, or state corruption), whereas incorrect or suboptimal model outputs that do not terminate execution are often tolerated or manually corrected, and thus less frequently reported as bugs. As a result, system-level failures that directly impact usability and workflow continuity are more prominently represented in issue reports than model behavior errors that primarily affect output quality. 

\textbf{\textit{Actionable design and testing implications.}}
Our findings point to several practical ways to design and test AI coding tools.

First, the interactions among LLMs, tools, and execution environments should be explicitly specified, validated, and continuously maintained. From a software engineering perspective, building AI coding tools introduces a substantially expanded set of artifacts, such as tool schemas, prompt templates, environment assumptions, and execution logs, all of which require systematic management and evolution. In addition, we also observe that many API and configuration failures stem from fragmentation issues, such as unexpected API formats, version mismatches, or incompatible runtime environments, which place significant stress on testing and validation. Proactively checking these conditions before execution can prevent cascading failures, avoid incorrect follow-up actions, and reduce user confusion. For example, AI coding tools could dynamically inspect users’ environments and automatically adapt or select compatible tools and configurations accordingly. 
Second, execution feedback should be clear and reliable for both users and models. Many failures attributed to the tool were, in fact, caused by hidden errors or missing feedback from earlier command executions, which emphasizes the importance of proper logging and traceability. Providing clear and structured execution feedback helps both users and models understand what occurred, preventing incorrect attribution of failures to the model and supporting more effective debugging and workflow recovery. 
Third, our results suggest that integration and scenario-based testing are essential. A single wrong assumption, such as an unsupported runtime setup, can affect multiple parts of the system before showing up as a user-facing bug.
Finally, tools should clearly indicate when execution feedback or system state is unreliable. Without such signals, models may act on incorrect information and produce wrong outputs. Simple indicators of invalid or uncertain state can help models pause, retry, or ask for clarification, improving robustness and user trust. 


==> sections/related.tex <==
\section{Related Works}
\label{sec:related}

==> tabs/bugtype-stage.tex <==
\begin{table*}[t]
\centering
\caption{Bug types that occur in different system execution stages.}
\label{tab:bug_type_stage_relation}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{lrrrrrrr}
\toprule
\textbf{Bug Type} & \makecell{\textbf{Tool/API}\\\textbf{Orchestration}} & \makecell{\textbf{Command Execution}\\\textbf{\& Monitoring}} & \makecell{\textbf{User Interface}\\\textbf{\& Interaction}} & \makecell{\textbf{State \& Memory}\\\textbf{Management}} & \makecell{\textbf{Prompt Engineering}\\\textbf{\& Context}\\\textbf{Management}} & \makecell{\textbf{LLM Reasoning}\\\textbf{Planning}}\\
\midrule
Functionality & 1431 & 947  & 563  & 317 & 214 & 246 \\
Usability     & 537  & 464  & 584  & 213 & 159 & 192 \\
Reliability   & 842  & 560  & 86   & 252 & 81  & 92  \\
Compatibility & 497  & 389  & 150  & 18  & 3   & 4   \\
Security      & 244  & 54   & 5    & 24  & 5   & 10  \\
Performance   & 117  & 98   & 23   & 67  & 20  & 13  \\
UI            & 5    & 8    & 250  & 5   & 2   & 2   \\
\textbf{Total} & \textbf{3673} & \textbf{2520} & \textbf{1661} & \textbf{896} & \textbf{484} & \textbf{559} &  \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> tabs/rootcause_locations.tex <==
\begin{table*}[t!]
\centering
\caption{Root cause categories across architectural layers.}
\vspace{-0.1in}
\label{tab:root_cause_vs_layer}
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrr}
\toprule
\textbf{Root Cause Category} &
\textbf{Tool / API Orchestration} &
\textbf{Command Execution \& Monitoring} &
\textbf{User Interface \& Interaction} &
\textbf{State \& Memory Management} &
\textbf{LLM Reasoning Planning} &
\textbf{Prompt Engineering \& Context Management} \\
\midrule

API \& Integration Errors
& 139 (16.8\%) & 23 (2.8\%) & 23 (2.8\%) & 46 (5.6\%) & 515 (62.3\%) & 80 (9.7\%) \\

Configuration \& Setup
& 177 (28.9\%) & 24 (3.9\%) & 37 (6.0\%) & 56 (9.1\%) & 235 (38.3\%) & 84 (13.7\%) \\

User Interaction \& UI
& 74 (17.2\%) & 13 (3.0\%) & 14 (3.3\%) & 28 (6.5\%) & 93 (21.6\%) & 208 (48.4\%) \\

Environment \& Platform Compatibility
& 163 (40.3\%) & 12 (3.0\%) & 20 (5.0\%) & 17 (4.2\%) & 105 (26.0\%) & 87 (21.5\%) \\

AI Logic \& Behavior
& 55 (14.3\%) & 131 (34.0\%) & 36 (9.4\%) & 24 (6.2\%) & 107 (27.8\%) & 32 (8.3\%) \\

Performance \& Resource Limits
& 86 (27.5\%) & 8 (2.6\%) & 20 (6.4\%) & 44 (14.1\%) & 121 (38.7\%) & 34 (10.9\%) \\

Command Execution \& Parsing
& 116 (44.3\%) & 8 (3.1\%) & 16 (6.1\%) & 15 (5.7\%) & 74 (28.2\%) & 33 (12.6\%) \\

State \& Context Management
& 35 (13.8\%) & 10 (4.0\%) & 30 (11.9\%) & 82 (32.4\%) & 77 (30.4\%) & 19 (7.5\%) \\

Code \& File Handling
& 54 (24.8\%) & 13 (6.0\%) & 20 (9.2\%) & 24 (11.0\%) & 71 (32.6\%) & 36 (16.5\%) \\

Permissions \& Security
& 64 (40.0\%) & 4 (2.5\%) & 3 (1.9\%) & 16 (10.0\%) & 57 (35.6\%) & 16 (10.0\%) \\




\bottomrule
\end{tabular}
}
\end{table*}

==> tabs/sentiment.tex <==
\begin{table}[t]
  \centering
  \caption{Sentiment distribution by forum category}
  \label{tab:sentiment_by_category}
  \scriptsize
  \setlength{\tabcolsep}{4pt} % tighten column spacing
  \begin{tabular}{lrrrrr}
    \toprule
    Forum Category & Very neg. & Neg. & Neutral & Pos. & Very pos. \\
    \midrule
    Bug Reports      & 255 (26.23\%) & 697 (97.21\%)  & 20 (2.79\%)   & 0             & 0             \\
    Feature request  & 59 (6.43\%)   & 514 (15.16\%)  & 1205 (41.90\%)& 1652 (98.86\%)& 19 (0.55\%)   \\
    Feedback         & 127 (13.83\%) & 458 (49.89\%)  & 197 (21.46\%) & 93 (10.13\%)  & 43 (4.68\%)   \\
    Discussion       & 707 (8.97\%)  & 3211 (40.75\%) & 3211 (40.75\%)& 631 (8.00\%)  & 119 (1.51\%)  \\
    How to           & 40 (2.70\%)   & 435 (29.37\%)  & 856 (57.80\%) & 133 (8.98\%)  & 17 (1.15\%)   \\
    \bottomrule
  \end{tabular}
\end{table}

==> tabs/severity.tex <==
\begin{table}[t]
  \centering
  \caption{Severity of posts by forum category}
  \label{tab:sentiment_by_category}
  \begin{tabular}{lrrrrr}
    \toprule
    Forum Category & Critical & High & Medium & Low \\
    \midrule
    Bug Reports      & 82 & 337 & 426  & 127 \\
    Feature Requests & 10  & 382 & 1661 & 1396 \\
    Feedback         & 25 & 221 & 339  & 333 \\
    Discussions      & 163 & 1550 & 2599 & 3567 \\
    How To           & 7 & 155 & 569  & 750 \\
    \bottomrule
  \end{tabular}
\end{table}
